ConsistentFeature: A Plug-and-Play Component for Neural Network Regularization

Over-parameterized neural network models often lead to significant performance discrepancies between training and test sets, a phenomenon known as overfitting. To address this, researchers have proposed numerous regularization techniques tailored to various tasks and model architectures. In this paper, we introduce a simple perspective on overfitting: models learn different representations in different i.i.d. datasets. Based on this viewpoint, we propose an adaptive method, ConsistentFeature, that regularizes the model by constraining feature differences across random subsets of the same training set. Due to minimal prior assumptions, this approach is applicable to almost any architecture and task. Our experiments show that it effectively reduces overfitting, with low sensitivity to hyperparameters and minimal computational cost. It demonstrates particularly strong memory suppression and promotes normal convergence, even when the model has already started to overfit. Even in the absence of significant overfitting, our method consistently improves accuracy and reduces validation loss.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> warmup.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/cvpr_result_full/ablation/warm_valloss.jpg}  % 替换为图片路径
    \caption{The Effect of Different Warm-up Steps on the Method
It is worth noting that even when the model has started overfitting before the intervention of our method, our approach is still able to return it to normal convergence.}  % 图片的标题
    \label{fig:warm_up_depracted}  % 图片的标签，用于引用
\end{figure}
